OWLAx: A Protege Plugin to Support Ontology Axiomatization through Diagramming

Once the conceptual overview, in terms of a somewhat informal class diagram, has been designed in the course of engineering an ontology, the process of adding many of the appropriate logical axioms is mostly a routine task. We provide a Protege plugin which supports this task, together with a visual user interface, based on established methods for ontology design pattern modeling.

==> conclusion.tex <==
% \section{Conclusions}\label{sec:conclusion}

% Conclusions

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

